SmoothOut: Smoothing Out Sharp Minima to Improve Generalization in Deep Learning

In Deep Learning, Stochastic Gradient Descent (SGD) is usually selected as a training method because of its efficiency; however, recently, a problem in SGD gains research interest: sharp minima in Deep Neural Networks (DNNs) have poor generalization; especially, large-batch SGD tends to converge to sharp minima. It becomes an open question whether escaping sharp minima can improve the generalization. To answer this question, we propose SmoothOut framework to smooth out sharp minima in DNNs and thereby improve generalization. In a nutshell, SmoothOut perturbs multiple copies of the DNN by noise injection and averages these copies. Injecting noises to SGD is widely used in the literature, but SmoothOut differs in lots of ways: (1) a de-noising process is applied before parameter updating; (2) noise strength is adapted to filter norm; (3) an alternative interpretation on the advantage of noise injection, from the perspective of sharpness and generalization; (4) usage of uniform noise instead of Gaussian noise. We prove that SmoothOut can eliminate sharp minima. Training multiple DNN copies is inefficient, we further propose an unbiased stochastic SmoothOut which only introduces the overhead of noise injecting and de-noising per batch. An adaptive variant of SmoothOut, AdaSmoothOut, is also proposed to improve generalization. In a variety of experiments, SmoothOut and AdaSmoothOut consistently improve generalization in both small-batch and large-batch training on the top of state-of-the-art solutions.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

==> experiments_sharpness.tex <==
\subsection{Sharpness and Robustness Analyses}
\label{sec:exp-sharpness-analyses}

Compare with ICLR and show sharpness in figures and metrics

Compare with NIPS and visualize using Hao Li's method


robust to image noise, weight quantization and adversarial attack?

show training accuracy is lower and explain why


show the accuracy is robust to the hyperparameter and explain it.

sensitivity analysis of hyperparameters

==> sensitivity_analyses.tex <==
\section{Sensitivity Analyses}
\label{supp:sens_analyses}

\begin{figure*}
	\centering
	\includegraphics[width=2.\columnwidth]{figures/cifar100_sharpness_test-crop.pdf}
	\caption{Notation:``SB'': Small Batch ($256$); ``LB'': Large Batch ($5000$); ``accu.'': accuracy.
		(a) loss and accuracy vs. $\alpha$, which controls $\bm{w}$ along the direction from SB minimum ($\bm{w}_f$) to LB minimum ($\bm{w}_s$);
		(b) loss and accuracy under influence of different strengths of noise. Dataset: CIFAR-100. Network: $C_3$. The optimizer is Adam with $0.001$ initial learning rate.}
	\label{fig:cifar100_sharpness_test}
\end{figure*}


\begin{figure*}
	\centering
	\includegraphics[width=2.\columnwidth]{figures/cifar_resnet_sharpness_test-crop.pdf}
	\caption{
		Loss and accuracy of ResNet-44 under influence of different strengths of noise on (a) CIFAR-10 and (b) CIFAR-100. The optimizer is SGD with momentum $0.9$.
	Notation:``SB'': Small Batch ($128$); ``LB'': Large Batch ($2048$ for CIFAR-10 and $1024$ for CIFAR-100); ``accu.'': accuracy.}
	\label{fig:cifar_resnet_sharpness_test}
\end{figure*}

==> sharpness_analyses.tex <==
\section{Sharpness Visualization}
\label{supp:sharpness_analyses}

\begin{figure*}[h]
	\centering
	\includegraphics[width=2.\columnwidth]{figures/cifar10_shallow_base_sout-crop.pdf}
	\caption{Sharpness of baseline and \sout{} in (a) ``SB'' training and (b) ``LB'' training of $C_1$.}
	\label{fig:cifar10_base_sout}
\end{figure*}

\begin{figure*}[h]
	\centering
	\includegraphics[width=2.\columnwidth]{figures/mnist_f1_base_sout-crop.pdf}
	\caption{Sharpness of baseline and \sout{} in (a) ``SB'' training and (b) ``LB'' training of $F_1$.}
	\label{fig:mnist_f1_base_sout}
\end{figure*}

==> tables/dnns.tex <==
\begin{table*}
  \caption{Baseline models.}
  \label{tab:dnns}
  \centering
  \resizebox{.85\textwidth}{!}{
  	\begin{tabular}{cccccccccr}
  		\toprule
  		DNN & Dataset & \begin{tabular}{@{}c@{}}Data \\ augment\end{tabular} &  Optimizer & Epochs & \begin{tabular}{@{}c@{}}Learning \\ rate\end{tabular} & GBN & \begin{tabular}{@{}c@{}}Batch \\ size\end{tabular} & Accuracy & \begin{tabular}{@{}c@{}}$(\mathcal{C}_{\epsilon}, A)$- \\ sharpness\end{tabular}\\
  		\midrule
  		   \multirow{2}{*}{$F_1$~(Keskar~\etal{}~\cite{keskar2016large})\textsuperscript{$\dagger$}}  & \multirow{2}{*}{MNIST} & \multirow{2}{*}{No} &  \multirow{2}{*}{Adam} & \multirow{2}{*}{$200$} & \multirow{2}{*}{$0.001$} & \multirow{2}{*}{No} & $256$ & $98.49\%$ & $0.0000$\\
  		   &  &  &  & & & & $6000$ & $98.01\%$ & $57.8246$\\
  		   \cmidrule{1-10}
  		   \multirow{2}{*}{$C_1$~(Keskar~\etal{}~\cite{keskar2016large})\textsuperscript{$\dagger$}}  & \multirow{2}{*}{ CIFAR-10} & \multirow{2}{*}{No} &  \multirow{2}{*}{Adam} & \multirow{2}{*}{$200$} & \multirow{2}{*}{$0.001$} & \multirow{2}{*}{No} & $256$ & $79.67\%$ & $27.7448$\\
  		   &  &  &  & & & & $5000$ & $77.30\%$ & $117.8266$\\
  		   \cmidrule{1-10}  		   
  		   \multirow{2}{*}{$C_3$~(Keskar~\etal{}~\cite{keskar2016large})\textsuperscript{$\dagger$}}  & \multirow{2}{*}{ CIFAR-100} & \multirow{2}{*}{No} & \multirow{2}{*}{Adam} & \multirow{2}{*}{$200$} & \multirow{2}{*}{$0.001$} & \multirow{2}{*}{No} & $256$ & $47.99\%$ & $23.5103$ \\
  		   &  &  &  & & & & $5000$ & $44.37\%$ & $62.0682$ \\
  		   
  		   \cmidrule{1-10}
  		   \textit{ResNet44}~(He~\etal{}~\cite{Kaiming_ResNet_ICCV}) & \multirow{3}{*}{ CIFAR-10} & \multirow{3}{*}{Yes} & \multirow{3}{*}{Momentum} & \multirow{3}{*}{$200$} & $0.1$ & No & $128$ & $93.18\%$ & $132.3693$ \\
  		   \textit{ResNet44}~(He~\etal{}~\cite{Kaiming_ResNet_ICCV}) &  &  &  & & $0.1$ & No & $2048$ & $87.58\%$ & $459.1477$ \\
  		   \textit{ResNet44}~(Hoffer~\etal{}~\cite{hoffer2017train})\textsuperscript{$\dagger$} &  &  &  & & $0.4$ & Yes & $2048$ & $89.24\%$ & $252.0197$ \\
  		   
  		   \cmidrule{1-10}
  		   \textit{ResNet44}~(He~\etal{}~\cite{Kaiming_ResNet_ICCV}) & \multirow{3}{*}{ CIFAR-100} & \multirow{3}{*}{Yes} & \multirow{3}{*}{Momentum} & \multirow{3}{*}{$200$} & $0.1$ & No & $128$ & $70.26\%$& $0.0000$ \\
  		   \textit{ResNet44}~(He~\etal{}~\cite{Kaiming_ResNet_ICCV}) &  &  &  & & $0.1$ & No & $1024$ & $64.67\%$ & $203.7407$ \\
  		   \textit{ResNet44}~(Hoffer~\etal{}~\cite{hoffer2017train})\textsuperscript{$\dagger$} &  &  &  & & $0.283$ & Yes & $1024$ & $67.23\%$ & $140.4747$ \\
  		   
  		   \cmidrule{1-10}
  		   \textit{AlexNet}~(Krizhevsky~\etal{}~\cite{Alex_NIPS2012_4824}) & \multirow{2}{*}{ ImageNet} & \multirow{2}{*}{Yes} & \multirow{2}{*}{Momentum} & \multirow{2}{*}{$60$} & $0.01$ & No & $256$ & $56.15\%$ & $595.9811$ \\
  		   \textit{AlexNet}~(Hoffer~\etal{}~\cite{hoffer2017train})\textsuperscript{$\dagger$} &  &  &  & & $0.113$ & Yes & $16384$ & $47.64\%$ & $623.0147$ \\
  		   
  		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  		
  		
  		\bottomrule 	
  		\multicolumn{10}{l}{\textsuperscript{$\dagger$} Models that are targeted on to close generalization gap by \sout{}. }	
  		
  	\end{tabular}
  }
%\vspace{-12pt}
\end{table*} 

==> tables/sharpness-study.tex <==
\begin{table*}
  \caption{Sharpness reduction and generalization improvement for DNNs in~\cite{keskar2016large}.}
  \label{tab:sharpness-study}
  \centering
  \resizebox{.85\textwidth}{!}{
  	\begin{tabular}{cccccccr}
  		\toprule
  		DNN & Dataset &  Optimizer & Epochs & \begin{tabular}{@{}c@{}}Learning \\ rate\end{tabular} & \begin{tabular}{@{}c@{}}Batch \\ size\end{tabular} & Accuracy & \begin{tabular}{@{}c@{}}$(\mathcal{C}_{\epsilon}, A)$- \\ sharpness\end{tabular}\\
  		\midrule
  		   \multirow{2}{*}{$F_1$}  & \multirow{2}{*}{MNIST} &  \multirow{2}{*}{Adam} & \multirow{2}{*}{$200$} & \multirow{2}{*}{$0.001$} & $256$ & $98.49\%$ & $0.0000$\\
  		   &  &   & & & $6000$ & $98.01\%$ & $57.8246$\\
  		   \cmidrule{1-8}
  		   \multirow{2}{*}{$C_1$}  & \multirow{2}{*}{ CIFAR-10} &  \multirow{2}{*}{Adam} & \multirow{2}{*}{$200$} & \multirow{2}{*}{$0.001$} & $256$ & $79.67\%$ & $27.7448$\\
  		   &  &  &  & & $5000$ & $77.30\%$ & $117.8266$\\
  		   \cmidrule{1-8}  		   
  		   \multirow{2}{*}{$C_3$}  & \multirow{2}{*}{ CIFAR-100}  & \multirow{2}{*}{Adam} & \multirow{2}{*}{$200$} & \multirow{2}{*}{$0.001$} & $256$ & $47.99\%$ & $23.5103$ \\
  		   &  &  &  & & $5000$ & $44.37\%$ & $62.0682$ \\
  		\bottomrule 	
  	\end{tabular}
  }
%\vspace{-12pt}
\end{table*} 
